Democratizing Uncertainty Quantification

Uncertainty Quantification (UQ) is vital to safety-critical model-based analyses, but the widespread adoption of sophisticated UQ methods is limited by technical complexity. In this paper, we introduce UM-Bridge (the UQ and Modeling Bridge), a high-level abstraction and software protocol that facilitates universal interoperability of UQ software with simulation codes. It breaks down the technical complexity of advanced UQ applications and enables separation of concerns between experts. UM-Bridge democratizes UQ by allowing effective interdisciplinary collaboration, accelerating the development of advanced UQ methods, and making it easy to perform UQ analyses from prototype to High Performance Computing (HPC) scale. In addition, we present a library of ready-to-run UQ benchmark problems, all easily accessible through UM-Bridge. These benchmarks support UQ methodology research, enabling reproducible performance comparisons. We demonstrate UM-Bridge with several scientific applications, harnessing HPC resources even using UQ codes not designed with HPC support.

==> benchmarks/inference/analytic-banana.tex <==
\subsubsection{Analytic Banana Benchmark}

This benchmark consists of an analytically defined PDF $\pi : \mathbb{R}^2 \rightarrow \mathbb{R}$ resembling the shape of a banana (see \cref{fig:analytic-banana}). It is based on a transformed normal distribution. The variance may be adjusted.

\begin{table}[h!]
  \centering
  \begin{tabular}{ccp{3cm}}
  \toprule
  Mapping & Dimensions & Description \\
  \midrule
  input  & [2] & Coordinates $\theta \in \mathbb{R}^2$ \\
  output & [1] & Log PDF $\pi$ evaluated at $\theta$ \\
  \bottomrule
  \end{tabular}
\caption{\it Properties of the Analytic Banana benchmark.}
\end{table}

Supported features of this benchmark are: Evaluate.

\begin{table}[h!]
  \centering
  \begin{tabular}{cccp{3cm}}
  \toprule
  Config & Type & Default & Description \\
  \midrule
  a & double & 2.0 & Transformation parameter \\
  b & double & 0.2 & Transformation parameter \\
  scale & double & 1.0 & Scaling factor applied to the underlying normal distribution's variance \\
  \bottomrule
  \end{tabular}
\caption{\it Configuration parameters the for Analytic Banana benchmark.}
\label{tbl:config_benchmarkname}
\end{table}

\begin{figure}
  \centering
     \includegraphics[width=0.49\textwidth]{Images/analytic-banana-samples.png}
     \includegraphics[width=0.49\textwidth]{Images/analytic-banana-contour.png}
      \caption{\it Samples drawn from the distribution defined through the PDF $\pi$, and their corresponding contour.}
\label{fig:analytic-banana}
\end{figure}

\todo[inline]{Move the four figures of analytic densities into one, should be cleaner}

We begin with a normally distributed random variable
$$Z \sim \mathcal{N}\left(\begin{pmatrix} 0 \\ 4 \end{pmatrix}, \text{scale} \begin{pmatrix} 1.0 & 0.5\\ 0.5 & 1.0 \end{pmatrix}\right),$$
and denote its PDF by $f_Z$.

In order to reshape the normal distribution, define a transformation $T : \mathbb{R}^2 \rightarrow \mathbb{R}^2$

$$ T(\theta) := \begin{pmatrix} \theta_1 / a \\ a \theta_2 + a b (\theta_1^2 + a^2) \end{pmatrix}. $$

Finally, the benchmark log PDF is defined as

$$ \log(\pi(\theta)) := \log(f_Z(T(\theta))). $$


==> benchmarks/inference/analytic-donut.tex <==
\subsubsection{Analytic Donut Benchmark}

This benchmark consists of an analytically defined PDF $\pi : \mathbb{R}^2 \rightarrow \mathbb{R}$ resembling the shape of a donut (see \cref{fig:analytic-donut}).

\begin{table}[h!]
  \centering
  \begin{tabular}{ccp{3cm}}
  \toprule
  Mapping & Dimensions & Description \\
  \midrule
  input  & [2] & Coordinates $\theta \in \mathbb{R}^2$ \\
  output & [1] & Log PDF $\pi$ evaluated at $\theta$ \\
  \bottomrule
  \end{tabular}
\caption{\it Properties of the Analytic Donut benchmark.}
\end{table}

Supported features of this benchmark are: Evaluate, Gradient, ApplyJacobian.

\begin{table}[h!]
  \centering
  \begin{tabular}{cccp{3cm}}
  \toprule
  Config & Type & Default & Description \\
  \midrule
  - & - & - & - \\
  \bottomrule
  \end{tabular}
\caption{\it Configuration parameters for the Analytic Donut benchmark.}
\end{table}

\begin{figure}
  \centering
     \includegraphics[width=0.49\textwidth]{Images/analytic-donut-samples.png}
     \includegraphics[width=0.49\textwidth]{Images/analytic-donut-contour.png}
      \caption{\it Samples drawn from the distribution defined through the PDF $\pi$, and their corresponding contour.}
\label{fig:analytic-donut}
\end{figure}

The PDF $\pi$ is defined as

$$ \pi(\theta) := - \frac{(\| \theta \| - r)^2}{\sigma^2}, $$

where $r = 2.6$ and $\sigma^2 = 0.033$.

The implementation then returns the log PDF $\log(\pi(\theta))$.


==> benchmarks/inference/analytic-funnel.tex <==
\subsubsection{Analytic Funnel Benchmark}

This benchmark consists of an analytically defined PDF $\tau : \mathbb{R}^2 \rightarrow \mathbb{R}$ resembling the shape of a funnel (see \cref{fig:analytic-funnel}).

\begin{table}[h!]
  \centering
  \begin{tabular}{ccp{3cm}}
  \toprule
  Mapping & Dimensions & Description \\
  \midrule
  input  & [2] & Coordinates $\theta \in \mathbb{R}^2$ \\
  output & [1] & Log PDF $\pi$ evaluated at $\theta$ \\
  \bottomrule
  \end{tabular}
\caption{\it Properties of the Analytic Funnel benchmark.}
\end{table}

Supported features of this benchmark are: Evaluate, Gradient, ApplyJacobian.

\begin{table}[h!]
  \centering
  \begin{tabular}{cccp{3cm}}
  \toprule
  Config & Type & Default & Description \\
  \midrule
  - & - & - & - \\
  \bottomrule
  \end{tabular}
\caption{\it Configuration parameters for the Analytic Funnel benchmark.}
\end{table}

\begin{figure}
  \centering
     \includegraphics[width=0.49\textwidth]{Images/analytic-funnel-samples.png}
     \includegraphics[width=0.49\textwidth]{Images/analytic-funnel-contour.png}
      \caption{\it Samples drawn from the distribution defined through the PDF $\pi$, and their corresponding contour.}
\label{fig:analytic-funnel}
\end{figure}

First, define a helper function

$$ f(\theta,m,s) := - \frac12 \log(2 \pi) - \log(s) - \frac12 ((\theta-m)/s)^2. $$

Now, the output log PDF is defined as

$$ \log(\tau(\theta)) := f(\theta_1, 0, 3) + f(\theta_2, 0, \exp(\frac12 \theta_1)). $$


==> benchmarks/inference/analytic-gaussian-mixture.tex <==
\subsubsection{Analytic Gaussian Mixture Benchmark}

This benchmark consists of an analytically defined PDF $\pi : \mathbb{R}^2 \rightarrow \mathbb{R}$ consisting of a Gaussian mixture (see \cref{fig:analytic-gaussian-mixture}).

\begin{table}[h!]
  \centering
  \begin{tabular}{ccp{3cm}}
  \toprule
  Mapping & Dimensions & Description \\
  \midrule
  input  & [2] & Coordinates $\theta \in \mathbb{R}^2$ \\
  output & [1] & Log PDF $\pi$ evaluated at $\theta$ \\
  \bottomrule
  \end{tabular}
\caption{\it Properties of the Analytic Gaussian Mixture benchmark.}
\end{table}

Supported features of this benchmark are: Evaluate, Gradient, ApplyJacobian.

\begin{table}[h!]
  \centering
  \begin{tabular}{cccp{3cm}}
  \toprule
  Config & Type & Default & Description \\
  \midrule
  - & - & - & - \\
  \bottomrule
  \end{tabular}
\caption{\it Configuration parameters for the Analytic Funnel benchmark.}
\end{table}

\begin{figure}
  \centering
     \includegraphics[width=0.49\textwidth]{Images/analytic-gaussian-mixture-samples.png}
     \includegraphics[width=0.49\textwidth]{Images/analytic-gaussian-mixture-contour.png}
      \caption{\it Samples drawn from the distribution defined through the PDF $\pi$, and their corresponding contour.}
\label{fig:analytic-gaussian-mixture}
\end{figure}

Let

$$X_1 \sim \mathcal{N}(\begin{pmatrix} -1.5 \\ -1.5 \end{pmatrix}, 0.8 I),$$
$$X_2 \sim \mathcal{N}(\begin{pmatrix} 1.5 \\ 1.5 \end{pmatrix}, 0.8 I),$$
$$X_3 \sim \mathcal{N}(\begin{pmatrix} -2 \\ 2 \end{pmatrix}, 0.5 I).$$

Denote by $f_{X_1}, f_{X_2}, f_{X_3}$ the corresponding PDFs.

The PDF $\pi$ is then defined as

$$ \pi(\theta) := \sum_{i=1}^3 f_{X_i}(\theta), $$

and the benchmark outputs $\log(\pi(\theta))$.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

